A Palm Calculus Approach to the Distribution of the Age of Information

A key metric to express the timeliness of status updates in latency-sensitive networked systems is the age of information (AoI), i.e., the time elapsed since the generation of the last received informative status message. This metric allows studying a number of applications including updates of sensory and control information in cyber-physical systems and vehicular networks as well as, job and resource allocation in cloud clusters. State-of-the-art approaches to analyzing the AoI rely on queueing models that are composed of one or many queuing systems endowed with service order, e.g., FIFO, LIFO, or last-generated-first-out order. A major difficulty arising in these analysis methods is capturing the AoI under message reordering when the delivery is non-preemptive and non-FIFO, i.e., when messages can overtake each other and the reception of informative messages may obsolete some messages that are underway. In this paper, we derive an exact formulation for the distribution of AoI in non-preemptive, non-FIFO systems where the main ingredients of our analysis are Palm calculus and time inversion. Owing to the rationality of the Laplace-Stieltjes transforms that are used in our approach, we obtain computable exact expressions for the distribution of AoI.

==> sections/reverse.old.tex <==
%!TEX root = ../main.tex
\section{Computing the Palm Distributions}
\label{sec:computing_palm_probabilities}


\subsection{Decomposition into Forward and Backward Components}
In order to compute the Palm PDF $f^\circ(x_0, t_1)$ we observe that the part on $x_0$ (the age) involves the past of $Z_t$ whereas the part on $t_1$ (time until a new arrival) involves the future of $Z_t$. This is captured by the following theorem.

 
\begin{theorem}
The joint PDF of both the age $x_0$ just after the informative message arrival \emph{and} the length of the cycle $t_1$ until the arrival of the next informative message is given by
\begin{align}
\label{eq:forward-backward2}
 f^\circ(x_0,t_1)= \sum_{(n',n) \mst 1\leq n+1\leq n'\leq I_{\max}} p^\circ_{n',n} g^\circ(x_0|n',n)h(t_1|n)
\end{align}
where
\begin{itemize}
  \item $p^\circ_{n',n}$ is the probability that an arbitrary message arrival 
happens at a transition $(n'\to n)$ of the Markov chain $Z_t$ and is given by
\begin{equation}
  p^\circ_{n',n} = \frac{p_{n'}}{\bar{N}} \; \ind{1\leq n+1\leq n'\leq I_{\max}}
\end{equation}
in the above, $\bar{N}:=\sum_{i=1}^{I_{\max}}i p_{i}$ is the stationary expectation of $Z_t$ and $p_i$ is given in \eqref{eq:steady_state_prob_chain_nr_msgs_underway};
  \item  $g^\circ(x_0|n',n)$ is the PDF of the Palm distribution of the age $x_0$ just after the informative message arrival given that the state of the Markov chain is $n'$ just before the arrival of the informative message and $n$ just after the arrival, where $n'\geq n+ 1$;
  \item  $h(t_1|n)$ is the stationary PDF of the time that will elapse from time $t$ until the next informative message arrives,  given that $Z_t=n$.

\end{itemize}
 \end{theorem}
The proof exploits the Markov property of $Z_t$, which expresses that the future depends on the past only through the present state.
 \begin{proof}
 

Define $f^\circ(x_0, t_1|n', n)$ as the joint PDF of the Palm distribution of
both the age $x_0$ just after the informative message arrival \emph{and}
the length of the cycle $t_1$ until the arrival of the next informative message, given that the state of the Markov chain is $n'$ just before the arrival of the informative message and $n$ just after the arrival, where $n'\geq n+ 1$.
 %age $x_0$ just after the arrival of an informative message arrived before time $t$ \emph{and} the time $t_1$ that will elapse from time $t$ until the next informative message arrives, given that $Z_t=n$.
It follows that the required PDF $f^\circ(x_0, t_1)$ is given by

\begin{align}
\label{eq:forward-backward}
 f^\circ(x_0,t_1)= \sum_{(n',n) \mst 1\leq n+1\leq n'\leq I_{\max}} p^\circ_{n',n} f^\circ(x_0, t_1|n',n)
\end{align}
where $p^\circ_{n',n}$  is the probability that an arbitrary message arrival 
happens at a transition $(n'\to n)$ of the Markov chain $Z_t$. By \cite[Thm 7.1.2]{boudec2011performance}, such a probability is given by

\begin{equation}
  p^\circ_{n',n} = \eta p_{n'} Q_{n',n}, \; \ind{1\leq n+1\leq n'\leq I_{\max}}
\end{equation}
where $\mathbf{1}_{\{\cdot\}}$ is the indicator function, equal to $1$ when the condition is true and $0$ otherwise, $p_{n'}$ is the stationary probability given in \eqref{eq:steady_state_prob_chain_nr_msgs_underway}, $Q_{n',n}$ is the transition rate in \eqref{eq:transition_rates_fwd_process} and $\eta$ is a normalizing constant.  Observe that $Q_{n',n}=\mu$, which gives $\eta^{-1}=\sum_{i=1}^{I_{\max}}i p_{i}:=\bar{N}$ where $\bar{N}$ is the stationary expectation of $Z_t$. It finally comes
\begin{equation}
  p^\circ_{n',n} = \frac{p_{n'}}{\bar{N}} \; \ind{1\leq n+1\leq n'\leq I_{\max}}
\end{equation}

\TBD{Because $p_nQ'_{n,n'}=p_{n'}Q_{n',n}$ this should be the same as \eqref{eq:normalization constant}...}

Let $g^\circ(x_0|n',n)$ denote the PDF of the Palm distribution of the age $x_0$ just after the informative message arrival given that the state of the Markov chain is $n'$ just before the arrival of the informative message and $n$ just after the arrival, where $n'\geq n+ 1$. 

Recall that
$h(t_1|n)$ denotes the stationary PDF of the time that will elapse from time $t$ until the next informative message arrives,  given that $Z_t=n$. By the Markov property, this is also the PDF of the Palm distribution of the time until the next informative message arrives given that the state of the Markov chain is $n'$ just before the arrival of the informative message and $n$ just after the arrival. Again by the Markov property,
$f(x_0, t_1|n'n)= g^\circ(x_0|n',n)h(t_1|n)$, which proves \eqref{eq:forward-backward2}.
\end{proof}

We next compute $h(t_1|n)$, which we call the forward component of \eqref{eq:forward-backward2}. The computation of the backward component $g^\circ(x_0|n',n)$ will involve a similar method plus a time-reversal argument.

\subsection{Computation of the Forward Component}

First, we will introduce the following lemma to calculate the Laplace-Stieltjes Transform (LST) of the time until the occurrence of the \emph{next transition of interest} in a continuous-time Markov chain $\{\tilde{Z}(t)\}_{t\in\mathbb{R_+}}$ conditioned on $Z_t=n$. The transitions of interest are defined by some subset $\tilde{\mathcal{F}}$ of $E\times E$, where $E\subseteq \mathbb{N}$ is the state-space of the Markov chain.

\begin{lemma}\label{lemma:LST_of_1st_event_forward_component_given_state_n}
Consider a time-homogeneous, continuous-time Markov chain $(Z_t)_{t\in\mathbb{R_+}}$ with state space $E\subseteq \Nats$
and with transition rates $Q_{n,n'}$;
let $\tilde{d}_{n}=\sum_{n'\in E}Q_{n,n'}$ denote the sum of all outgoing rates from state $n$ and
assume that $\tilde{d}_{n}>0$ for all $n\in E$. Let $\tilde{\mathcal{F}}\subseteq E$ such that
$Q_{n,n'}> 0$
for all $(n,n')\in \tilde{\mathcal{F}}$.

Call $\tilde{Y}_t$ the time that will elapse from $t$ until the next jump in $\tilde{\mathcal{F}}$ of the Markov chain, i.e.
$\tilde{Y}_t =\inf\{s> 0, (Z_{(t+s)^-},Z_{(t+s)^+})\in \tilde{\mathcal{F}}\}$.
% a set of transitions of interest $\tilde{\mathcal{F}}\coloneqq \{(i,j)\} \subseteq \{(i,j)\}_{Q_{i,j}>0}$.
% Fix some arbitrary time $t$ and call $\tilde{Y}_t$ the time that will elapse from $t$ until the next transition of interest conditioned on $\tilde{Z}(t)=n$.
The conditional LST of $\tilde{Y}_t$ given that $Z_t=n$, denoted as $\tilde{f}_{n}(\nu)$, satisfies
% \begin{align}
% &\tilde{f}_{n}(\nu) \coloneqq \E\left[e^{-\nu \tilde{Y}_t} | Z_t=n\right] \nonumber\\
% &= \frac{\tilde{d}_{n}}{\tilde{d}_{n}+ \nu}\left(\sum_{\substack{n',\\(n,n')\notin\tilde{\mathcal{F}}}} \tilde{f}_{n'}(\nu) \frac{Q_{n,n'}}{\tilde{d}_{n}}+ \sum_{\substack{n',\\(n,n')\in\tilde{\mathcal{F}}}} \frac{Q_{n,n'}}{\tilde{d}_{n}}\right) ,
% \label{eq:LST_of_next_transition_of_interest}
% \end{align}
\begin{align}
&\tilde{f}_{n}(\nu) \coloneqq \E\left[e^{-\nu \tilde{Y}_t} | Z_t=n\right] \nonumber\\
&= \frac{1}{\tilde{d}_{n}+ \nu}\left(\sum_{\substack{n',\\(n,n')\notin\tilde{\mathcal{F}}}} \tilde{f}_{n'}(\nu) Q_{n,n'}+ \sum_{\substack{n',\\(n,n')\in\tilde{\mathcal{F}}}} Q_{n,n'}\right).
\label{eq:LST_of_next_transition_of_interest}
\end{align}
%where
%$\tilde{S}_t$ is the time until the next transition out of state $Z_t$ and
%$\tilde{d}_{n}=\sum_{n'\in E}Q_{n,n'}$  denotes the sum of all outgoing rates from state $n$.
\end{lemma}
%
\begin{proof}
\TBD{See if proof cannot be simplified by considering the time until next visit to a subset of states}
%
Fix some arbitrary time $t$ and define $\tilde{S}_t$ as the time until the next transition (of interest or not) out
of state $Z_t$ and let $ N'_t\coloneqq Z_{t+\tilde{S}_t}$ denote the next state. It is known \cite{gillespie1976general} that, conditional to $Z_t=n$, $N'_t$ and $\tilde{S}_t$ are independent, the distribution of $\tilde{S}_t$ is exponential with rate
$\tilde{d}_{n}$ and the distribution of $N'_t$ is given by $\P(N'_t=n'| Z_t=n)=\frac{Q_{n,n'}}{\tilde{d}_n}$. It follows that
%
\begin{equation}
\P\left[N'_t=n'| Z_t=n,\tilde{S}_t=s\right]=\frac{Q_{n,n'}}{\tilde{d}_n}
\label{eq:gillespie}
\end{equation}
and
\begin{equation}
\E\left[e^{-\nu \tilde{S}_t}\right] = \frac{\tilde{d}_{n}}{\tilde{d}_{n}+ \nu}
\label{eq:gillespie2}
\end{equation}

Also let $\tilde{R}_t$ denote the residual time from the next transition until the next transition of interest, i.e. $\tilde{R}_t=0$ whenever $(Z_t,N'_t)\in \tilde{\mathcal{F}}$ and
otherwise %$\tilde{R}_t=\inf\{s\geq 0, (Z_{(t+\tilde{S}_t+s)^-},Z_{(t+\tilde{S}_t+s)^+})\in \tilde{\mathcal{F}}\}$. It follows that
$\tilde{R}_t=\tilde{Y}_{t+\tilde{S}_t}$. Hence
%
%
%  To obtain the conditional LST in \eqref{eq:LST_of_next_transition_of_interest} we fix some arbitrary time $t$ and decompose $\tilde{Y}_t$, i.e., the time that will elapse from $t$ until the next transition of interest, %conditioned on $Z_t=n$
% into
%express the time until the next arrival of an informative message given state $Z_t=n$ as
\begin{equation}
\tilde{Y}_t = \tilde{S}_t + \tilde{R}_t
\label{eq:Y_first_departure}
\end{equation}
%where $\tilde{S}_t$ is the time until the next transition (of interest or not) out of state $Z_t$ and $\tilde{R}_t$ denotes the residual time from the next transition until the next transition of interest (so that $\tilde{R}_t=0$ whenever the next transition is a transition of interest). We also let $ N'_t\coloneqq Z_{t+\tilde{S}_t}$ denote the next state.
%

By conditioning on $\tilde{S}_t=s$ we can write
\begin{align}
&\E\left[e^{-\nu \tilde{Y}_t} | Z_t=n,\tilde{S}_t=s\right] \nonumber\\
&= e^{-\nu s}\E\left[e^{-\nu \tilde{R}_t} | Z_t=n,\tilde{S}_t=s\right]
\label{eq:Y_lst_1}
\end{align}

By conditioning with respect to $N'_t$ in the latter term and applying \eqref{eq:gillespie} we obtain
\begin{align}
&\E\left[e^{-\nu \tilde{R}_t} | Z_t=n,\tilde{S}_t=s\right] \nonumber\\
&= \sum_{n'\in E}\left(\E\left[e^{-\nu \tilde{R}_t} | Z_t=n,\tilde{S}_t=s, N'_t=n'\right]\times \right.\nonumber\\
&\left.\P\left[N'_t=n'| Z_t=n,\tilde{S}_t=s\right]\right)\nonumber\\
&=\sum_{n'\in E}\left(\E\left[e^{-\nu \tilde{R}_t} | Z_t=n,\tilde{S}_t=s, N'_t=n'\right]\frac{Q_{n,n'}}{\tilde{d}_n}\right)
\label{eq:Y_lst_1b}
\end{align}


Now if $(n,n')\in \tilde{\mathcal{F}}$ then $\tilde{R}_t=0$ hence
\begin{equation}
\E\left[e^{-\nu \tilde{R}_t} |Z_t=n,\tilde{S}_t=s, N'_t=n'\right]=1  \mbox{ if } (n,n')\in \tilde{\mathcal{F}}
\label{eq:Y_lst_1c}
\end{equation}


% By the Markov property, the future of the Markov chain depends on the history only via the current state, i.e.
% \begin{align}
% &\E\left[e^{-\nu \tilde{Y}_{t+\tilde{S}_t}} | Z_t=n,\tilde{S}_t=s, N'_t=n'\right] \nonumber\\
% &=
% \E\left[e^{-\nu \tilde{Y}_{t+s}} | N'_t=n'\right]=  \E\left[e^{-\nu \tilde{Y}_{t+s}} | Z_{t+s}=n'\right]
% \end{align}
Else, i.e. if $(n,n')$ is not in $\tilde{\mathcal{F}}$, $\tilde{R}_t=\tilde{Y}_{t+\tilde{S}_t}$ is the time that remains
to elapse until the next transition of interest; by the Markov property,
the future of the Markov chain depends on the history only via the current state, i.e.
\begin{align}
&\E\left[e^{-\nu \tilde{Y}_{t+\tilde{S}_t}} | Z_t=n,\tilde{S}_t=s, N'_t=n'\right] \nonumber\\
&
=\E\left[e^{-\nu \tilde{Y}_{t+s}} | N'_t=n'\right]=  \E\left[e^{-\nu \tilde{Y}_{t+s}} | Z_{t+s}=n'\right] \nonumber\\
&=\tilde{f}_{n'}(\nu)
\label{eq:Y_lst_1d}
\end{align}
where the last equality is because the Markov chain is time-homogeneous.

Combining \eqref{eq:Y_lst_1} with \eqref{eq:Y_lst_1b}-\eqref{eq:Y_lst_1d} gives
\begin{align}
&\E\left[e^{-\nu \tilde{Y}_t} | Z_t=n,\tilde{S}_t=s\right]\nonumber\\
&= e^{-\nu s}\left(\sum_{\substack{n',\\(n,n')\notin\tilde{\mathcal{F}}}} \tilde{f}_{n'}(\nu) \frac{Q_{n,n'}}{\tilde{d}_{n}}+ \sum_{\substack{n',\\(n,n')\in\tilde{\mathcal{F}}}} \frac{Q_{n,n'}}{\tilde{d}_{n}}\right)
\label{eq:Y_lst_1f}
\end{align}
%where we used the set of transitions of interest $\tilde{\mathcal{F}}$ and the definition of the sum of all outgoing rates from state $n$ as $\tilde{d}_{n}$.
By the law of total expectation we can now write
\begin{align}
&\tilde{f}_{n}(\nu) = \E\left[e^{-\nu \tilde{Y}_t} | Z_t=n\right] \nonumber\\
&=\E\left[\E\left[e^{-\nu \tilde{Y}_t} | Z_t=n,\tilde{S}_t\right]\right] \nonumber\\
&= \E\left[e^{-\nu \tilde{S}_t}\right]\left(\sum_{\substack{n',\\(n,n')\notin\tilde{\mathcal{F}}}} \tilde{f}_{n'}(\nu) \frac{Q_{n,n'}}{\tilde{d}_{n}}+ \sum_{\substack{n',\\(n,n')\in\tilde{\mathcal{F}}}} \frac{Q_{n,n'}}{\tilde{d}_{n}}\right)
\label{eq:LST_of_next_transition_of_interest2}
\end{align}
Using \eqref{eq:gillespie2} completes the proof.
\end{proof}
\vspace{5pt}

Now we can use Lem.~\ref{lemma:LST_of_1st_event_forward_component_given_state_n} to calculate the stationary PDF $h(t_1|n)$ of the time that will elapse from a fixed time $t$ until the next informative message arrives conditioned on $Z_t=n$.
%This computation uses the Markov property of $Z_t$, as illustrated by the Lemma.
The set of transitions of interest is $\tilde{\mathcal{F}}\coloneqq \{(i,j)\}_{i>j}$, i.e. the transitions associated with the arrival of informative messages. % and $\tilde{Y}_t$ as the time that will elapse from $t$ until the next arrival of an informative message.
The transition rates $Q_{i,j}$ are given in \eqref{eq:transition_rates_fwd_process} and
%We also used the definition of the sum of all outgoing rates from state $n$ as
$\tilde{d}_{n}= \lambda \mathbf{1}_{\{n<I_{\max}\}} + \mu n$, where $\mathbf{1}_{\{\cdot\}}$ is the indicator function, equal to $1$ when the condition is true and $0$ otherwise.

%
%Fix some arbitrary time $t$ and call $\tilde{Y}_t$ the time that will elapse from $t$ until the next arrival of an informative message, so that $h(t_1|n)$ is the conditional PDF of $\tilde{Y}_t$ given that $Z_t=n$.
%%Also call $T^+_t$ the time until the next transition of the Markov chain. We have ...

The Laplace-Stieltjes Transform of $h(t_1|n)$ continues to be denoted by $\tilde{f}_{n}(\nu)$; the application of Lem.~\ref{lemma:LST_of_1st_event_forward_component_given_state_n} gives:
\begin{align}
\tilde{f}_{n}(\nu) = \frac{1}{\tilde{d}_{n}+ \nu} \left[  n \mu +  \lambda\tilde{f}_{n+1}(\nu)\right].
%\tilde{f}_{n}(\nu) = \frac{\tilde{d}_{n}}{\tilde{d}_{n}+ \nu} \left[  \frac{n \mu}{\tilde{d}_{n}} +  \frac{\lambda}{\tilde{d}_{n}} \tilde{f}_{n+1}(\nu)\right].
\label{eq:LST_of_next_arrival_given_state_nprime}
\end{align}
%where we used the transition rates $Q_{n,n'}$ from \eqref{eq:transition_rates_fwd_process} in the last line.
%inspecting the \emph{forward component} as follows:
%We regard a state $n$ and express the time until the next arrival of an informative message
%%(in the forward process given state $n'$)
%as
%\begin{equation}
%Z_{n} = R_{n} + Z_{n'}
%\label{eq:Z_first_departure}
%\end{equation}
%where $R_{n}$ is exponentially distributed with parameter $\tilde{d}_{n}\coloneqq \lambda \mathbf{1}_{\{n<I_{\max}\}} + \mu n$, i.e., the sum of all outgoing rates from state $n$ with the indicator function $\mathbf{1}_{\{\cdot\}}$ and the variable  $Z_{n'}$ is given as
%\begin{equation}
%Z_{n'} = \begin{cases}
% 0&\text{for any \emph{down} transition with rate $n \mu$}\\
%Z_{n+1}&\text{for the \emph{up} transition with rate $\lambda$}
%\end{cases}
%\label{eq:Z'_first_departure}
%\end{equation}
%Now, we can write for the conditional LST of the time until the next arrival given state $n$ as
\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{./gfx/sample_path_jumps3}
  \caption{A sample path of the number of non-obsolete messages under way given the system model from Sect.~\ref{sec:system_model}. Looking at the forward process: The downward jumps mark the arrival of informative messages at the receiver which make previous messages obsolete. As messages depart in batches of random sizes in this model the waiting time of the freshest message of the batch corresponds to the age value set upon the arrival of that message at the receiver.}
  \label{fig:sample_path_jumps}
\end{figure}
%
%\begin{align}
%\tilde{f}_{n}(\nu)  = \frac{\tilde{d}_{n}}{\tilde{d}_{n}+ \nu} \left[  \frac{n \mu}{\tilde{d}_{n}} +  \frac{\lambda}{\tilde{d}_{n}} \tilde{f}_{n+1}(\nu)\right].
%\label{eq:LST_of_next_arrival_given_state_nprime}
%\end{align}
This recursive relation can be rewritten using matrix notation as
\begin{equation}
%(\theta \mt{I} + \mt{D})
\mt{(\nu I + \tilde{D}) \tilde{f} = \pmb{\bar{\mu}} + \bar{\Lambda} \tilde{f}}
\label{eq:LST_of_next_arrival_given_state_nprime_matrix_recursive}
\end{equation}
with the identity matrix $\mt{I}$, the vectors  $\mt{\tilde{f}}= [\tilde{f}_{0}(\nu),\dots,\tilde{f}_{I_{\max}}(\nu)]\T$, and $\pmb{\bar{\mu}} = [0,\mu,2\mu\dots,I_{\max}\mu]\T$, and the matrices $\mt{\tilde{D}} \coloneqq \diag (\tilde{d}_0,\tilde{d}_1,\dots,\tilde{d}_{I_{\max}})$,
and
\begin{align}
\pmb{\bar{\Lambda}}
\coloneqq
\begin{bmatrix}
  \mathbf{0} &   \lambda& \hdots& \mathbf{0}  \\
\vdots &  \ddots& \lambda& \vdots \\
\vdots& \ddots& \ddots &\lambda\\
\mathbf{0} & \hdots & \mathbf{0}&\mathbf{0}
\end{bmatrix}.
\label{eq:definition_of_Lambda_bar}
\end{align}
Now we can directly solve for the conditional LSTs as
\begin{equation}
%(\theta \mt{I} + \mt{D})
\mt{\tilde{f} = (\nu I + \tilde{D} - \bar{\Lambda})^{-1} \pmb{\bar{\mu}} }
\label{eq:LST_of_next_arrival_given_state_nprime_matrix}
\end{equation}
%The computation of $h(t_1|n)$ is directly obtained from the $n$th component of the inverse Laplace transform vector of  \eqref{eq:LST_of_next_arrival_given_state_nprime_matrix}.


\subsection{Computation of the Backward Component}

Recall that $g^\circ(x_0|n',n)$ denotes the PDF of the Palm distribution of the age $x_0$ just after the informative message arrival
given that the state of the Markov chain is $n'$ just before the arrival of the informative message and $n$ just after the arrival, where $n'\geq n+ 1$.
 %given that the state of the Markov chain just after the arrival is $n$. %the stationary PDF of the age $x_0$ just after the last informative message arrived before time $t$ given that $Z_t=n$.
%With the terminology of queueing theory as in Sect.~\ref{sec:underlying_model}, $g^\circ(x_0|n)$ refers to the time elapsed
since the arrival of the freshest message in the served batch.
%which corresponds to the age $x_0$ just after the informative message arrival.
For the computation of $g^\circ(x_0|n',n)$ we resort to time-reversal as this allows to use a similar method as for the forward component.

The time-reversed process $Z_t^r$ is defined by $Z_t^r=Z_{-t}$.
In a nutshell, time reversal allows us to change the underlying queueing model from Sect.~\ref{sec:underlying_model} into a FIFO queue where arrivals occur in message batches of random size while the server removes exactly \emph{one} message on each visit.
To illustrate this, consider the sample path shown in Fig.~\ref{fig:sample_path_jumps} in the reverse time direction. 
%The original process $Z_t$ has individual arrivals and batch departures, whereas the time-reversed process $Z_t^r$ has batch arrivals and individual departures. 

It is shown in \cite{Kelly:Reversibility2011} [Section 1.7] that if $Z_t$ is endowed with its stationary probability, then the
time-reversed process is also a time-homogeneous continuous time Markov chain with same state space and same stationary probability,
but with different transitions rates. Specifically, by \cite{Kelly:Reversibility2011} [Theorem 1.12] the transition rates $Q'_{i,j}$
for $Z_t^r$ depend on the transition rates of the original Markov process \eqref{eq:transition_rates_fwd_process} and its stationary
distribution \eqref{eq:steady_state_prob_chain_nr_msgs_underway}. We obtain $Q'_{i,i-1} =\lambda_{i}'$ for $i=1...I_{\max}$, $Q'_{i,j} =\mu_{ij}'$ for $i=0...I_{\max}-1,i<j\leq I_{\max}$ and $Q'_{i,j} =0$ otherwise, with
%
%
%
\begin{equation}
\lambda_i' = \begin{cases}
\frac{i}{i+1}\left(\lambda + (i+1) \mu\right) &\text{for $1\leq i < I_{\max}$}\\ \\
I_{\max} \mu &\text{for $i = I_{\max}$}
\end{cases}
\label{eq:lambda_prime}
\end{equation}
and
\begin{equation}
\mu_{ij}' = \begin{cases}
 \frac{(j+1) \mu \lambda^{j-i}}{(i+1)\prod\limits_{k=i+2}^{j+1}\left(\lambda + k\mu\right)}&\text{for $j \neq I_{\max}$}\\ \\
\frac{\lambda^{I_{\max}-i}}{(i+1)\prod\limits_{k=i+2}^{I_{\max}}\left(\lambda + k\mu\right)}&\text{for $j = I_{\max}$}
\end{cases}
\label{eq:mu_prime}
\end{equation}
for $0\leq i< I_{\max}$. The derivation of \eqref{eq:lambda_prime}, \eqref{eq:mu_prime} is given in the appendix.

\TBD{We now have the mapping:\\
\begin{tabular}{c|c|c|c|c}
old & $n-k$ & $n$ & $n-k+1$ & $k$\\\hline
new & $n$ & $n'$ & $n+1$ & $n'-n$
\end{tabular}
}

In $Z_t$, upon serving a batch of messages, the sojourn time of the freshest message of that batch is the age of that particular informative message. In $Z^r_t$, this is given by the sojourn time of the $(n-k+1)$st message of an arriving batch of size $k\leq n$. In $Z^r_t$, the 
arrival of a batch corresponds to a transition $n\to n'$ with $n'\geq n+1$ and the size of the arriving batch is $k=n'-n$. It follows that, for $n'\geq n+ 1$, $g^\circ(x_0|n',n)$ can be re-interpreted as the PDF of the time from now until the $(n+1)$st departure of $Z^r_t$, given that $Z^r_t$ is doing a transition $n\to n'$ now.  
Since $Z^r_t$ is also Markov, we can apply the Markov property and obtain that this is 
simply the PDF of the time from now until the $(n+1)$st departure of $Z^r_t$ 
given that $Z^r_t=n'$. For $n+1=1$ this is the conditional PDF of the time until a next departure, which is exactly the problem that is solved in Lemma~\ref{lemma:LST_of_1st_event_forward_component_given_state_n}, and which we now extend as follows (the proof is similar and is not given). 



\begin{lemma}\label{lemma:LST_of_all_events_forward_component_given_state_n}
Consider a time-homogeneous, continuous-time Markov chain $(\tilde{Z}_t)_{t\in\mathbb{R_+}}$ with state space $E\subseteq \Nats$
and with transition rates $\tilde{Q}_{n,n'}$;
let $\tilde{d}_{n}=\sum_{n'\in E}\tilde{Q}_{n,n'}$ denote the sum of all outgoing rates from state $n$ and
assume that $\tilde{d}_{n}>0$ for all $n\in E$. Let $\tilde{\mathcal{F}}\subseteq E$ such that
$\tilde{Q}_{n,n'}> 0$
for all $(n,n')\in \tilde{\mathcal{F}}$.

For $k\geq 1$, call $\tilde{Y}^k_t$ the time that will elapse from $t$ until the $k$th jump in $\tilde{\mathcal{F}}$ of the Markov chain, i.e.
$\tilde{Y}^1_t =\inf\{s\geq 0, (\tilde{Z}_{(t+s)^-},\tilde{Z}_{(t+s)^+})\in \tilde{\mathcal{F}}\}$ and for $k\geq 2$, $\tilde{Y}^k_t =\inf\{s> Y^{k-1}, (\tilde{Z}_{(t+s)^-},\tilde{Z}_{(t+s)^+})\in \tilde{\mathcal{F}}\}$.
% a set of transitions of interest $\tilde{\mathcal{F}}\coloneqq \{(i,j)\} \subseteq \{(i,j)\}_{\tilde{Q}_{i,j}>0}$.
% Fix some arbitrary time $t$ and call $\tilde{Y}_t$ the time that will elapse from $t$ until the next transition of interest conditioned on $\tilde{Z}(t)=n$.
The conditional LST of $\tilde{Y}^k_t$ given that $\tilde{Z}_t=n$, denoted as $\tilde{f}_{n,k}(\theta)$, satisfies, for $k\geq 1$:
% \begin{align}
% &\tilde{f}_{n}(\theta) \coloneqq \E\left[e^{-\theta \tilde{Y}_t} | \tilde{Z}_t=n\right] \nonumber\\
% &= \frac{\tilde{d}_{n}}{\tilde{d}_{n}+ \theta}\left(\sum_{\substack{n',\\(n,n')\notin\tilde{\mathcal{F}}}} \tilde{f}_{n'}(\theta) \frac{\tilde{Q}_{n,n'}}{\tilde{d}_{n}}+ \sum_{\substack{n',\\(n,n')\in\tilde{\mathcal{F}}}} \frac{\tilde{Q}_{n,n'}}{\tilde{d}_{n}}\right) ,
% \label{eq:LST_of_next_transition_of_interest}
% \end{align}
\begin{align}
&\tilde{f}_{n,k}(\theta) = \frac{1}{\tilde{d}_{n}+ \theta} \times \nonumber\\
&\left(\sum_{\substack{n',\\(n,n')\notin\tilde{\mathcal{F}}}} \tilde{f}_{n',k}(\theta) \tilde{Q}_{n,n'}+ \sum_{\substack{n',\\(n,n')\in\tilde{\mathcal{F}}}} \tilde{f}_{n',k-1}(\theta)\tilde{Q}_{n,n'}\right).
\label{eq:LST_of_next_transition_of_interest}
\end{align}
where $\tilde{f}_{n,0}(\theta)=1$ by convention.
%$\tilde{S}_t$ is the time until the next transition out of state $\tilde{Z}_t$ and
%$\tilde{d}_{n}=\sum_{n'\in E}\tilde{Q}_{n,n'}$  denotes the sum of all outgoing rates from state $n$.
\end{lemma}
%



 

% To obtain the Palm distribution of the age just after the arrival of an informative message at time $t_+$, we first consider the time-reversed process $Z_t^r$ conditioned on $\{(Z_{t_+}^r=n-k, Z_{t}^r=n)\}$, i.e., the reverse-time Markov chain jumps from state $n-k$ to state $n$ at time $t$.
% Note that the arrival of informative messages corresponds to the set of transitions $\{(n',n)\}_{n'<n}$, with rates $Q'_{n',n}$. 
% Taking the transition $\{(n-k,n)\}$ with rate $k\geq 1$ and $Q'_{n-k,n}$, we observe that it corresponds to the arrival of one informative message that obsoletes exactly $k-1$ older messages.
% To obtain the age of this informative message we define the set of transitions of interest as $\mathcal{F}\coloneqq \{(i,j)\}_{i>j}$, i.e., the transitions corresponding to departures in the time-reversed process. 
% Given that the time-reversed process jumps from state $Z_{t_+}^r=n-k$ to state $Z_t^r=n$ at time $t$, we consider the time $Y_t$ that will elapse from time $t$ until the departure
% of the $n-k+1^{st}$ message. 
% This time is the age of the informative message that arrives at the transition $\{(Z_{t_+}^r=n-k, Z_{t}^r=n)\}$. 

%\TBD{We should compress a bit from here, there is now no need to do $k=1$ separately.}

Let $f_{n',k}(\theta)$ be the LST of the time from now until the $k$th departure of $Z^r_t$ 
given that $Z^r_t=n'$, so that the LST of $g^\circ(x_0|n',n)$ is
$f_{n', n+1}$. We now apply Lemma~\ref{lemma:LST_of_all_events_forward_component_given_state_n} to the Markov chain $Z^r_t$ to compute $f_{n',k}(\theta)$ and obtain:


% . We now compute apply Lemma~\ref{lemma:LST_of_all_events_forward_component_given_state_n} gives the set of recursive equations:


% In the following, we will calculate the LST of the time $Y_t$ that will elapse until the $k$th departure given the jump $\{(n-k,n)\}$. We denote this conditional LST by $f_{n,k}(\theta)$.

% As it is more instructive we first start by illustrating the calculation for the LST of the time until the \emph{first} departure $f_{n,1}(\theta)$ before generalizing the computation to the $k$th departure.





% \TBD{The following is not well explained and needs more accuracy. }
% As we are interested in the distribution of the age of the informative messages $g^\circ(x_0|n)$, we seek an expression that describes the time until the departure of a specific message of the batch that corresponds to the age given the state $n$.
% Recall the observation on the forward process $Z_t$ from above that upon serving a batch of messages the sojourn time of the freshest message of that batch is the age of that particular informative message.
% %Hence, in forward direction this corresponds to the consideration that
% In particular, given $n$ messages in the queue and that a batch of size $k\leq n$ messages is served then the sojourn time that corresponds to the age is of the $n-k+1$st message.
% %is the one for the message for which we need to go arrivals back.
% %If a batch of size $k=n$ messages is served then the sojourn time of interest is of the message that entered the queue last.
% Hence, to obtain the LST of the age at the times when informative messages arrive we calculate first the conditional LST of the $n-k+1$st departure given state $n$. We combine this result with \eqref{eq:LST_of_next_arrival_given_state_nprime_matrix} into \eqref{eq:forward-backward2}.


% First, we calculate the transition rates of the reversed process $Z_t^r$.
% %We finally use this result to calculate the LST of the age at any point in time $f(x)$ using the inversion formula \eqref{eq:f_age_fct_of_pdf_at_arrival}.
% Given this time reversal argument we obtain for $Z_t^r$ the Markov chain with the transition rates $\lambda_i'$ $\mu_{ij}'$.
% Given the transition rates of the Markov process \eqref{eq:transition_rates_fwd_process} and the steady state distribution given through \eqref{eq:steady_state_prob_chain_nr_msgs_underway} we obtain the transition rates for the reversed process
%  using [Theorem 1.12] from \cite{Kelly:Reversibility-2011} as $Q'_{i,i-1} :=\lambda_{i}'$ for $i=1...I_{\max}$, $Q'_{i,j} :=\mu_{ij}'$ for $i=0...I_{\max}-1,i<j\leq I_{\max}$ and $Q'_{i,j} :=0$ otherwise. For the given Markov process we calculate $\lambda_{i}',\mu_{ij}'$ as follows
% %
% \begin{equation}
% \lambda_i' = \begin{cases}
% \frac{i}{i+1}\left(\lambda + (i+1) \mu\right) &\text{for $1\leq i < I_{\max}$}\\ \\
% I_{\max} \mu &\text{for $i = I_{\max}$}
% \end{cases}
% \label{eq:lambda_prime}
% \end{equation}
% and
% \begin{equation}
% \mu_{ij}' = \begin{cases}
%  \frac{(j+1) \mu \lambda^{j-i}}{(i+1)\prod\limits_{k=i+2}^{j+1}\left(\lambda + k\mu\right)}&\text{for $j \neq I_{\max}$}\\ \\
% \frac{\lambda^{I_{\max}-i}}{(i+1)\prod\limits_{k=i+2}^{I_{\max}}\left(\lambda + k\mu\right)}&\text{for $j = I_{\max}$}
% \end{cases}
% \label{eq:mu_prime}
% \end{equation}
% for $0\leq i< I_{\max}$. The derivation of \eqref{eq:lambda_prime}, \eqref{eq:mu_prime} is given in the appendix.
%In the following, we utilize this model to calculate the conditional Laplace-Stieltjes Transform (LST) of the age given the arrival of a message at the receiver.
%As the process $X_t$ is constructed by considering some selected transitions of the Markov chain $\{\tilde{Z}(t)\}_{t\in\mathbb{R_+}}$ that describes the reversed time process it is sufficient to show that this Markov chain is stationary to show that $X_t$ is also stationary. The Markov chain of the reversed process with the transition rates $Q'_{i,j}$ described above is irreducible and hence stationary.

%Next, we provide the distribution of the time until the departure of the last message of a batch.


%\subsubsection{LST of the time until the first departure}
%Here, we adapt the expressions in Lem.~\ref{lemma:LST_of_1st_event_forward_component_given_state_n} to the reversed process and follow the exact same steps as in the derivation of \eqref{eq:LST_of_next_arrival_given_state_nprime} to obtain
%Similar to the derivation in \eqref{eq:Y_first_departure}-\eqref{eq:LST_of_next_arrival_given_state_nprime} we express the time that will elapse from $t$ until the next departure given that $Z_t^r=n$ as
%\begin{equation}
%Y_t = \tilde{S}_t+\tilde{R}_t
%\label{eq:Y_first_departure_reverse}
%\end{equation}
%\begin{align}
%f_{n,1}(\theta) = \frac{1}{d_n+ \theta} \left[  \lambda_n' +  \sum\limits_{j>n}\mu_{nj}' f_{j,1}(\theta)\right]
%\label{eq:LST_of_next_departure_given_state_n}
%\end{align}
%
\begin{eqnarray}
f_{n',1}(\theta) \left[d_{n'} +\theta\right]&=& \lambda_{n'} + \sum\limits_{j>n'} \mu_{n',j}' f_{j,1}(\theta)\label{eq:LST_of_next_departure_given_state_n_v2a}\\
f_{n',k}(\theta) \left[d_{n'} +\theta\right]&=& \lambda_{n'} f_{n',k-1}(\theta)+ \sum\limits_{j>n'} \mu_{n',j}' f_{j,1}(\theta)
\label{eq:LST_of_next_departure_given_state_n_v2b}
\end{eqnarray}
for $0\leq n'\leq I_{\max}$ and $k\geq 2$.
% , where we use \eqref{eq:lambda_prime}-\eqref{eq:mu_prime} for the and the definition $d_{n}\coloneqq \sum_{n'}Q'_{n,n'}$.
% Note that the time  $\tilde{S}_t$ until the next transition out of state $n$  is exponentially distributed with parameter $d_n = \lambda_n'+\sum\limits_{j>n}\mu_{nj}'$.
%, i.e., the sum of all outgoing rates from state $n$.
%
%We can express the time until the next departure given state $n$ as
%\begin{equation}
%Y_n = T_n + Y_n'
%\label{eq:Y_first_departure}
%\end{equation}
%where $T_n$ is exponentially distributed with parameter $d_n \coloneqq \lambda_n'+\sum\limits_{j>n}\mu_{nj}'$, i.e., the sum of all outgoing rates from state $n$ and the variable  $Y_n'$ is given as
%\begin{equation}
%Y_n' = \begin{cases}
% 0&\text{for the \emph{down} transition with rate $\lambda_n'$}\\
%Y_j&\text{for any \emph{up} transition with rate $\mu_{nj}'$, $j>n$}\nonumber
%\end{cases}
%\label{eq:Y'_first_departure}
%\end{equation}
%Hence, we can write for the conditional LST of the time until the first departure given state $n$
%\begin{align}
%f_{n,1}(\theta) = \frac{d_n}{d_n+ \theta} \left[  \frac{\lambda_n'}{d_n} +  \sum\limits_{j>n}\frac{\mu_{nj}'}{d_n} f_{j,1}(\theta)\right]
%\label{eq:LST_of_next_departure_given_state_n}
%\end{align}
%where we first separate the LST of $T_n$ and $Y_n'$ and evaluate the expectation.
%

%Now, we can rewrite \eqref{eq:LST_of_next_departure_given_state_n} for every state $0\leq n\leq I_{\max}$ as
%\begin{equation}
%f_{n,1}(\theta) \left[d_n +\theta\right]= \lambda_n' + \sum\limits_{j>n} \mu_{nj}' f_{j,1}(\theta).
%\label{eq:LST_of_next_departure_given_state_n_v2}
%\end{equation}

We use the following matrix notation: $\mt{D} \coloneqq \diag (d_0,d_1,\dots,d_{I_{\max}})$, 
$\mt{f}_{\cdot,k} = [f_{0,k}(\theta),\dots,f_{I_{\max},k}(\theta)]\T$,
%$\mt{f}_{\cdot,1} = [f_{0,1}(\theta),\dots,f_{I_{\max},1}(\theta)]\T$,
 $\pmb{\lbar'} = [0,\lambda_1',\dots,\lambda_{I_{\max}}']\T$. $\mt{M}$ is the upper triangular matrix
%$\mt{M} \coloneqq \mt{\left[m_{ij}\right\}}$ such that $m_{ij} = 0$ for $i\geq j$
\begin{equation*}
\mt{M} = \begin{cases*}
\mu_{ij}'&\text{for $i < j$}\\
0&\text{for $i \geq j$}
\end{cases*}
%\label{eq:matrix_M_triangular}
\end{equation*}
and 
$\pmb{\Lambda}$ is the matrix with $\lambda_n'$ on the subdiagonal defined by
\begin{align}
\pmb{\Lambda}
\coloneqq
\begin{bmatrix}
  \mathbf{0} &  \hdots& \hdots& \mathbf{0}  \\
\lambda_1' & \ddots & & \vdots \\
\vdots& \ddots& \ddots &\vdots\\
\mathbf{0} & \hdots & \lambda_{I_{\max}}'&\mathbf{0}
\end{bmatrix}.
\label{eq:definition_of_Lambda}
\end{align}
%



for $i,j \in \{0,1,\dots,I_{\max}\}$, 
We can rewrite the recursive relation of the conditional LST in  \eqref{eq:LST_of_next_departure_given_state_n_v2a} as
\begin{equation}
%(\theta \mt{I} + \mt{D})
\mt{(\theta I + D) f_{\cdot,1} = \pmb{\lbar'} + M f_{\cdot,1}}
\label{eq:LST_of_next_departure_given_state_n_matrix_recursive}
\end{equation}
The previous equation can be solved and we obtain:
\begin{equation}
%(\theta \mt{I} + \mt{D})
\mt{f_{\cdot,1} = (\theta I + D - M)^{-1} \pmb{\lbar'} }
\label{eq:LST_of_next_departure_given_state_n_matrix}
\end{equation}
%\begin{equation}
%f_n(\theta) = \frac{d_n}{\lambda_n'+\sum\limits_{j>n}\mu_{nj}' + \theta} \left[  \frac{\lambda_n'}{\lambda_n'+\sum\limits_{j>n}\mu_{nj}'} +  \sum\limits_{j>n}\frac{\mu_{nj}'}{\lambda_n'+\sum\limits_{j>n}\mu_{nj}'} f_j(\theta)\right]
%\label{eq:LT_of_next_departure_given_state_n}
%\end{equation}

%\begin{equation}
%f_n(\theta) \left[\lambda_n'+\sum\limits_{j>n}\mu_{nj}' + \theta\right]= \lambda_n' + \sum\limits_{j>n} \mu_{nj}' f_j(\theta)
%\label{eq:LST_of_next_departure_given_state_n_v2}
%\end{equation}

%\subsubsection{LST of the time until the $k$th departure}

%Next, we generalize the analysis from above to calculate the conditional LST for the time until the $k$th  departure with $k \in \{1,\dots,I_{\max}\}$ given state $n$. To this end, we introduce the following lemma:

%Similar to \eqref{eq:Y_first_departure} we can write
%\begin{equation}
%Y_{n,k} = T_n + Y_{n',k}
%\label{eq:Y_kth_departure}
%\end{equation}
%with
%{\small
%\begin{equation}
%Y_{n',k} = \begin{cases}
%Y_{n-1,k-1} &\text{for the \emph{down} transition with rate $\lambda_n'$}\\
%Y_{j,k}&\text{for any \emph{up} transition with rate $\mu_{nj}'$, $j>n$}
%\end{cases}
%\label{eq:Y'_kth_departure}
%\end{equation}
%}
%\noindent owing to the fact that the defined Markov chain is skip-free (see Fig.~\ref{fig:MC_fwd} for comparison and note the difference to the forward process).
%Similar to \eqref{eq:LST_of_next_departure_given_state_n_v2} the following Lemma expresses the conditional LST of the time until the $k$th departure given state $n$.




% \begin{lemma}\label{lemma:LST_of_kth_departure_given_state_n}
% Given a Markov chain $\{\tilde{Z}(t)\}_{t\in\mathbb{R_+}}$ that describes the reversed time process with transition rates \eqref{eq:lambda_prime} and \eqref{eq:mu_prime}. Given that the Markov chain is in state $n$ the Laplace-Stieltjes Transform of the time until the $k$th departure $f_{n,k}(\theta)$ is given through the recursion
% \begin{equation}
% f_{n,k}(\theta) \left[d_n +\theta\right]= \lambda_n'f_{n-1,k-1}(\theta) + \sum\limits_{j>n} \mu_{nj}' f_{j,k}(\theta).
% \label{eq:LST_of_kth_departure_given_state_n}
% \end{equation}
% \end{lemma}
% %
% \begin{proof}
% The proof of Lemma~\ref{lemma:LST_of_kth_departure_given_state_n} follows by the Markov property, the fact that $Z_t^{\tilde{r}}$ is downward skip-free and the observation that the time $Y_{t,k}$ that will elapse from $t$ until the $k$th departure given state $n$ can be split as $Y_{t,k} = \tilde{S}_t + R_{t,k}$ where ${S}_t$ is the time until the next transition out of state $Z_t^{\tilde{r}}$ and ${R}_t$ denotes the residual time until the $k$th departure after leaving state $Z_t^{\tilde{r}}$. Now by conditioning on $\tilde{S}_t=s$ similar to \eqref{eq:Y_lst_1} we obtain
% \begin{align}
% &\E\left[e^{-\theta {Y}_{t,k}} | Z_t^{\tilde{r}}=n,\tilde{S}_t=s\right] \nonumber\\
% &= e^{-\theta s}\Big(\mkern-18mu\sum_{\substack{n',\\(n,n')\notin{\mathcal{F}}}} \mkern-18mu{f}_{n',k}(\theta) \frac{Q'_{n,n'}}{{d}_{n}}+\mkern-18mu \sum_{\substack{n',\\(n,n')\in{\mathcal{F}}}}\mkern-18mu {f}_{n',k-1}(\theta) \frac{Q'_{n,n'}}{{d}_{n}}\Big)
% \label{eq:Y_lst_k}
% \end{align}
% where we used the set of transitions of interest as $\mathcal{F}\coloneqq \{(i,j)\}_{i>j}$.
% Note that a transition $(n,n') \in \mathcal{F}$ leads to the conditional LST ${f}_{n',k-1}$ of the time until the $k-1$\ts{st} departure given state $n'$.
% Now, by taking the law of total expectation and the transition rates for the reverse time process we obtain
% \begin{align}
% &\tilde{f}_{n,k}(\theta) = \E\left[e^{-\theta {Y}_{t,k}} | Z_t^{\tilde{r}}=n\right] \nonumber\\
% &=\E\left[\E\left[e^{-\theta \tilde{Y}_{t,k}} | Z_t^{\tilde{r}}=n,{S}_t\right]\right] \nonumber\\
% &= \E\left[e^{-\theta {S}_t}\right]\Big(\mkern-18mu\sum_{\substack{n',\\(n,n')\notin{\mathcal{F}}}} \mkern-18mu{f}_{n',k}(\theta) \frac{Q_{n,n'}}{{d}_{n}}+ \mkern-18mu\sum_{\substack{n',\\(n,n')\in{\mathcal{F}}}} \mkern-18mu{f}_{n',k-1}(\theta) \frac{Q_{n,n'}}{{d}_{n}}\Big)\nonumber\\
% &=\frac{{d}_{n}}{{d}_{n}+ \theta} \left[  \frac{\lambda_n'}{{d}_{n}}f_{n-1,k-1}(\theta) + \sum\limits_{j>n} \frac{\mu_{nj}'}{d_n} f_{j,k}(\theta). \right].
% \label{eq:LST_of_kth_arrival_given_state_nprime}
% \end{align}
% %
% %Here, $T_n$ is the time until the next transition out of state $n$ which is exponentially distributed with $d_n = \lambda_n'+\sum\limits_{j>n}\mu_{nj}'$, i.e., the sum of all outgoing rates from state $n$. Further, $Y_{n',k}$ is defined as either the time until the $k-1^{\text{st}}$ departure from state $n-1$ given that a departure occurred from state $k$ or recursively as the time until the $k$th departure from state $j$ given a transition upward with rate $\mu_{nj}'$ as in \eqref{eq:Y'_kth_departure}. Taking the Laplace transform on \eqref{eq:Y_kth_departure} with the definition of $Y_{n',k}$ we obtain the conditional LST in \eqref{eq:LST_of_kth_departure_given_state_n}.
% \end{proof}
%
Similarly, we can re-write \eqref{eq:LST_of_next_departure_given_state_n_v2b} as
% Next, we use the matrix notation $\mt{f}_{\cdot,k} = [f_{0,k}(\theta),\dots,f_{I_{\max},k}(\theta)]\T$ for $1\leq k\leq I_{\max}$ and the
% the matrix $\pmb{\Lambda}$ that is defined with $\lambda_n'$ on the subdiagonal as
% \begin{align}
% \pmb{\Lambda}
% \coloneqq
% \begin{bmatrix}
%   \mathbf{0} &  \hdots& \hdots& \mathbf{0}  \\
% \lambda_1' & \ddots & & \vdots \\
% \vdots& \ddots& \ddots &\vdots\\
% \mathbf{0} & \hdots & \lambda_{I_{\max}}'&\mathbf{0}
% \end{bmatrix}.
% \label{eq:definition_of_Lambda}
% \end{align}
% %
% We now apply Lemma~\ref{lemma:LST_of_all_events_forward_component_given_state_n} 
% to a general $k$ and obtain
\begin{equation}
%(\theta \mt{I} + \mt{D})
\mt{(\theta I + D) f_{\cdot,k} = \pmb{\Lambda}f_{\cdot,k-1} + M f_{\cdot,k}}
\label{eq:LST_of_only_kth_departure_given_state_n_matrix_recursive}
\end{equation}
for $k\geq 2$. %Note that for $k=1$ we already possess the form \eqref{eq:LST_of_next_departure_given_state_n_matrix_recursive}.
Now we can construct a block matrix form that takes \eqref{eq:LST_of_next_departure_given_state_n_matrix_recursive} as well as \eqref{eq:LST_of_only_kth_departure_given_state_n_matrix_recursive} to follow the form
%
\begin{align}
\scalemath{0.83}{
%(\theta \mt{I} + \mt{D})
\begin{bmatrix}
\mt{\theta I + D} &  & \mathbf{0}  \\
& \ddots & \\
\mathbf{0} & &  \mt{\theta I + D}
\end{bmatrix}
\begin{bmatrix}
\mt{f_{\cdot,1}} \\
\vdots \\
\mt{f_{\cdot,I_{\max}}}
\end{bmatrix}
=
\begin{bmatrix}
\pmb{\lbar'}  \\
\vdots \\
\mathbf{0}
\end{bmatrix}
+
\begin{bmatrix}
\mt{M} &  & \mathbf{0}  \\
\pmb{\Lambda} & \ddots & \\
\mathbf{0} &\pmb{\Lambda}  & \mt{M}
\end{bmatrix}
\begin{bmatrix}
\mt{f_{\cdot,1}} \\
\vdots \\
\mt{f_{\cdot,I_{\max}}}
\end{bmatrix}
}
\label{eq:LST_of_kth_departure_given_state_n_matrix_recursive}
\end{align}

We can directly find the vector of conditional LST as
\begin{align}
%(\theta \mt{I} + \mt{D})
\begin{bmatrix}
\mt{f_{\cdot,1}} \\
\vdots \\
\mt{f_{\cdot,I_{\max}}}
\end{bmatrix}
=
\begin{bmatrix}
\mt{\theta I + D-M} &  & \mathbf{0}  \\
\pmb{-\Lambda} & \ddots & \\
\mathbf{0} &\pmb{-\Lambda}  & \mt{\theta I + D-M}
\end{bmatrix} ^{-1}
\begin{bmatrix}
\pmb{\lbar'}  \\
\vdots \\
\mathbf{0}
\end{bmatrix}
\label{eq:LST_of_kth_departure_given_state_n_matrix}
\end{align}


Since the computation of \eqref{eq:LST_of_kth_departure_given_state_n_matrix} requires the inversion of a matrix of the order of $I_{\max}^2\times I_{\max}^2$ we show in the following how to calculate the conditional LST recursively from \eqref{eq:LST_of_kth_departure_given_state_n_matrix_recursive}.
We observe that $\mt{M- D  = Q' - \Lambda}$ where  $\mt{Q'}$ denotes the transition rate matrix of the continuous Markov chain associated with the reversed process $Z_t^r$.
We define $\mt{\Phi \coloneqq \theta I + D - M}$ and obtain the following recursion in block matrix form
\begin{align*}
%(\theta \mt{I} + \mt{D})
\begin{bmatrix}
\mt{\Phi} &  & &  \\
\pmb{-\Lambda} & \ddots & \mbox{\Large $\mathbf{0}$}&\\
\mathbf{0} & \ddots& \ddots & \\
\mathbf{0} & \mathbf{0} & \pmb{-\Lambda}  & \mt{\Phi}
\end{bmatrix}
\begin{bmatrix}
\mt{f_{\cdot,1}} \\
\vdots \\
\vdots \\
\mt{f_{\cdot,I_{\max}}}
\end{bmatrix}
=
\begin{bmatrix}
\pmb{\lbar'}  \\
\vdots \\
\vdots \\
\mathbf{0}
\end{bmatrix}
%\label{eq:LST_of_kth_departure_given_state_n_matrix_recursion_final}
\end{align*}
Now we obtain the conditional LST $\mt{f_{\cdot,n}}$ recursively with the initial condition
\begin{align}
\mt{f_{\cdot,1} = \Phi^{-1} \pmb{\lbar'}}
\label{eq:LST_of_1st_departure_given_state_n_initial_condition}
\end{align}
and for $k\geq 2$
\begin{align}
\mt{f_{\cdot,k} =  \Psi^{k-1}\Phi^{-1} \pmb{\lbar'}}
\label{eq:LST_of_kth_departure_given_state_n_rest_of_recursion}
\end{align}
where we used the shorthand notation $\mt{\Psi \coloneqq \Phi^{-1}\Lambda}$.



\begin{figure*}
\centering
  \begin{subfigure}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{./simulations/matlab/fig/ccdf_age_at_inform_arrival_lambda1_comparison_mu_05_1_2_max_msgs20_log_trace_len5.eps}
    \caption{}
    \label{fig:ccdf_age_at_inform_2}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{./simulations/matlab/fig/pdf_age_at_any_point_lambda1_mu_comparison_0.5_1_2_max_msgs20_log_trace_len5.eps}
    \caption{}
    \label{fig:pdf_age_at_anytime}
  \end{subfigure}
%  \hfill
%    \begin{subfigure}[b]{0.325\linewidth}
%    \includegraphics[width=\linewidth]{./simulations/matlab/fig/quantile_age_at_anytime_mu1_lambdastart0.1_lambdaend2_nr_lambda20_max_msgs20_log_trace_len5.eps}
%    \caption{}
%    \label{fig:quantile_age_anytime_I_20}
%  \end{subfigure}
 \caption{(a) CCDF of the age at the arrival times of informative messages for arrival rate $\lambda=1$ and varying OWD parameter $\mu$. $I_{\max} = 20$. (b) Probability density of the age $f(x)$ at any point in time obtained from \eqref{eq:f_age_fct_of_pdf_at_arrival} for $\lambda=1$ and varying OWD parameter $\mu$. $I_{\max} = 20$.}
\end{figure*}

\subsection{Computing $f^\circ(x_0, t_1)$}
We can now put together the forward and backward elements. Let 
$\hat{f}(\nu,\theta)$ denote the LST of $f^\circ(x_0,t_1)$, specifically
\begin{equation}
  \hat{f}(\nu,\theta):=\int_{0}^{\infty}\int_{0}^{\infty} f^\circ(x_0,t_1) e^{-\nu t_1} e^{-\theta x_0} dt_1 dx_0
\end{equation}
From \eqref{eq:forward-backward2} is comes
\begin{align}
\label{eq:joint_LST_x_t}
\int_{0}^{\infty}\int_{0}^{\infty} & f^\circ(x_0,t_1) e^{-\nu t_1} e^{-\theta x_0} dt_1 dx_0  \\
& =  \frac{1}{\eta}\sum\limits_{\substack{k,n \\ k\leq n}} p_{n-k}\mt{Q'(n-k,n)} f_{n,n-k+1}(\theta) \tilde{f}_{n-k}(\nu)\nonumber
\end{align}
where $\tilde{f}_{n-k}(\nu)$ resembles the conditional LST of the time until the next departure in the \emph{forward component} given state $n-k$.
The formulation \eqref{eq:joint_LST_x_t} reflects the terms in \eqref{eq:forward-backward2}, i.e., that the joint stationary PDF of the age and the time until the next arrival of an informative message are conditionally independent given state $n-k$. 




\section{Computing Age performance Metrics}
\TBD{This needs now to be aligned to the previous section.}
\subsection{Age distribution at arbitrary points in time}

To obtain the age distribution at any point in time we construct the PDF $f^\circ(x_0, t_1)$ from \eqref{eq:forward-backward2}. From the previous subsection we obtain the LST of the decomposed forward and backward components $\tilde{f}_{n-k}(\nu)$ and $f_{n,n-k+1}(\theta)$, respectively.
Next, we compute $p^\circ_n$, i.e., the probability that the state of the Markov chain is $n$ just after the arrival of an informative message.
To compute this we consider the backward component and use the set of transitions of interest $\mathcal{F'}\coloneqq \{(i,j)\}_{i<j}$, i.e., the transitions at the rates $\mu_{ij}'$.
Note that these transitions correspond to the arrival of informative messages.

Now, we can calculate the stationary probability $p^\circ_n$ as
\begin{align}
p_n^0 &= \frac{\sum\limits_{\substack{n'<n,\\(n',n)\in{\mathcal{F'}}}}\mkern-18mu p_{n'}Q'_{n',n}}{\sum\limits_{\substack{n',\\(n',n)\in{\mathcal{F'}}}}\mkern-18mu p_{n'}Q'_{n',n}} \\
&= \frac{1}{\eta}\sum_{k<n}p_{n-k} \mt{Q'(n-k,n)}
\label{eq:p_circ_n2}
\end{align}
%
where $p_{n-k}$ is the steady state probability from \eqref{eq:steady_state_prob_chain_nr_msgs_underway}, $\mt{Q'(n-k,n)}$ denotes the $(n-k,n)$ entry (transition rate $Q'_{n-k,n}$) of the transition rate matrix $\mt{Q'}$, and $\eta$ is normalization constant for the steady state probabilities $p_n$ by the aggregate transitions rates leading to the arrival of an informative message, i.e.,
\begin{align}
\eta = \sum_{n=0}^{I_{\max}-1} p_n \sum_{j>n} \mu_{nj}' .
\label{eq:normalization constant}
\end{align}
.
%\sum_{\substack{n',\\(n,n')\in{\mathcal{F}}}}


We can now obtain the distribution of the age at any point in time through the Palm inversion as given in \eqref{eq:f_age_fct_of_pdf_at_arrival}.
To this end we compute the LST of $f^\circ(x_0,t_1)$ after insertion into \eqref{eq:forward-backward2} as
\begin{align}
\label{eq:joint_LST_x_t}
\int_{0}^{\infty}\int_{0}^{\infty} & f^\circ(x_0,t_1) e^{-\nu t_1} e^{-\theta x_0} dt_1 dx_0  \\
& =  \frac{1}{\eta}\sum\limits_{\substack{k,n \\ k\leq n}} p_{n-k}\mt{Q'(n-k,n)} f_{n,n-k+1}(\theta) \tilde{f}_{n-k}(\nu)\nonumber
\end{align}
where $\tilde{f}_{n-k}(\nu)$ resembles the conditional LST of the time until the next departure in the \emph{forward component} given state $n-k$.
The formulation \eqref{eq:joint_LST_x_t} reflects the terms in \eqref{eq:forward-backward2}, i.e., that the joint stationary PDF of the age and the time until the next arrival of an informative message are conditionally independent given state $n-k$. 

\TBD{This should be clear from Section IV.A and should not be explained now. Also, it is too vague to be convincing.}
%For a better illustration this is sketched in Fig.~\ref{}.






Now, we proceed to the distribution of the age at any point in time by inserting the Palm joint density $f^\circ(x_0,t_1)$ that is obtained from the calculation of the inverse Laplace transform of the formulation \eqref{eq:joint_LST_x_t} for given $\lambda, \mu$ into  \eqref{eq:f_age_fct_of_pdf_at_arrival}.

\TBD{What is the result ? Shouldn't we say more as this is supposed to be the main outcome !}

\paragraph*{Remark} As all the Laplace-Stieltjes transforms encountered here are rational the distributions associated with them are matrix-exponential. This allows computing closed form results for the age distribution given $\lambda, \mu$.


\subsection{The expected age}

%Based on the calculation of the density function of the AoI at the arrival times of informative packets in \eqref{eq:LST_time_until_informative_msg} and the subsequent calculation of the AoI density from \eqref{eq:f_age_fct_of_pdf_at_arrival} we can directly obtain the expected AoI from \eqref{eq:expectation_test_fct_age} when setting the test function $\varphi$ as identity function.

To obtain the expected age we use the formulation of the age density given in \eqref{eq:f_age_fct_of_pdf_at_arrival}.
As illustrated above we obtain the density $f^\circ(x_0,t_1)$ by calculating the inverse Laplace transform of the formulation \eqref{eq:joint_LST_x_t} for given $\lambda, \mu$.
Calculating the expected age from the closed form density formulation obtained from \eqref{eq:f_age_fct_of_pdf_at_arrival} is, hence, straightforward.

%The compute the age density we require the density of the time between two informative messages which we denote $\tilde{f}'(x)$.
%In the following, we calculate the LST of $\tilde{f}'(x)$ in a similar fashion to the derivation of the age distribution at the arrival instances of informative messages above.
%
%Finally, we obtain the LST of the time between two informative messages with density $\tilde{f}'(x)$ as
%\begin{align}
%\int_{0}^{\infty} \tilde{f}'(v) e^{-\theta v} dv =  \frac{1}{\eta}\sum\limits_{\substack{k,n \\ k\leq n}} p_{n-k}\mt{Q(n-k,n)} \tilde{f}_{n}(\theta)
%\label{eq:LST_time_between_informative_msg}
%\end{align}
%Note the similarity of this expression to \eqref{eq:LST_time_until_informative_msg}. In a nutshell, we consider here the events of an arrival in the reversed process (i.e. an informative message) and calculate the distribution to the next arrival which is the next informative message.


To empirically obtain the average age from the event based simulation we utilize the Palm inversion formula \eqref{eq:palm_inversion_formula} with $\varphi$ set as identity function and $\lambda$ in  \eqref{eq:palm_inversion_formula}  replaced by $\lambda^\circ = \lambda (1 - p_{I_{\max}})$.
Hence we can write
    \begin{align}
    &E\left[X\right] = \lambda^\circ E^\circ\left[\int_{0}^{T_1}X_s ds \right] = \lambda^\circ E^\circ\left[\int_{0}^{T_1}A+s ~ds \right] \nonumber \\
    &= \lambda^\circ E^\circ\left[AT_1 + \frac{1}{2} T_1^2 \right] \nonumber \\
    &= \lambda^\circ E\left[A_n(T_{n+1}-T_n)\right]  + \frac{\lambda^\circ}{2} E\left[(T_{n+1}-T_n)^2 \right].
    \label{eq:plam_expectation}
  \end{align}
Here, $A_n$ is the age at the receiver just after the arrival of the $n$th informative message at the time point $T_n$.



\subsection{Age distribution at the arrival of informative messages}
Given the calculations above we can easily calculate the distribution of the age at the \emph{arrival instants of informative messages}.
This is directly obtained by computing the LST of the time until the departure of an informative message with density function $f^\circ(v)$ as
\begin{align}
\int_{0}^{\infty} f^\circ(v) e^{-\theta v} dv =  \frac{1}{\eta}\sum\limits_{\substack{k,n \\ k\leq n}} p_{n-k}\mt{Q'(n-k,n)} f_{n,n-k+1}(\theta) .
\label{eq:LST_time_until_informative_msg}
\end{align}
%
Note that the Laplace-Stieltjes transforms $f_{n,n-k+1}(\theta)$ utilized above are rational, hence, the distributions associated with them are matrix-exponential which renders $f^\circ(v)$ to be matrix-exponential.
For given $\lambda$ and $\mu$  we obtain $f^\circ(v)$ by calculating the inverse Laplace transform of the formulation above.

\begin{figure*}
\centering
  %\begin{subfigure}[b]{0.325\linewidth}
%    \includegraphics[width=\linewidth]{./simulations/matlab/fig/ccdf_age_at_inform_arrival_lambda1_mu0.25_0.5_1_2_4_max_msgs16_log_trace_len6.eps}
%    \caption{}
%    \label{fig:ccdf_age_at_inform_2}
%  \end{subfigure}
%  \hfill
  \begin{subfigure}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{./simulations/matlab/fig/mean_age_at_anytime_mu1_lambdastart0.1_lambdaend2_nr_lambda29_max_msgs20_log_trace_len5_no_relwork.eps}
    \caption{}
    \label{fig:mean_age_anytime_I_20}
  \end{subfigure}
  \hfill
    \begin{subfigure}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{./simulations/matlab/fig/quantile_age_at_anytime_mu1_lambdastart0.1_lambdaend2_nr_lambda20_max_msgs20_log_trace_len5.eps}
    \caption{}
    \label{fig:quantile_age_anytime_I_20}
  \end{subfigure}
 \caption{(a)  Expected age $E[X]$ obtained from simulations compared to the model in \eqref{eq:expectation_test_fct_age} with $\varphi$ being the identity function for $I_{\max}=20$ and $\mu=1$. (b) Quantiles of the age $P[X>x_{\varepsilon}]=\varepsilon$ obtained from integrating the age density in \eqref{eq:f_age_fct_of_pdf_at_arrival} for $I_{\max}=20$ and $\mu=1$.}
\end{figure*}
%
%\begin{figure}
%  \centering
%  \includegraphics[width=\linewidth]{./simulations/matlab/fig/ccdf_age_at_inform_arrival_lambda1_mu0.25_0.5_1_2_4_max_msgs16_log_trace_len6.eps}
%  \caption{Age at the arrival times of informative messages for arrival rate $\lambda=1$ and varying OWD parameter $\mu$. $I_{\max} = 16$. }
%  \label{fig:ccdf_age_at_inform_2}
%\end{figure}
%
%
%\begin{figure}
%  \centering
%  \includegraphics[width=\linewidth]{./simulations/matlab/fig/mean_age_at_anytime_mu1_lambdastart0.1_lambdaend2_nr_lambda29_max_msgs20_log_trace_len5_no_relwork.eps}
%  \caption{Expected age $E[X]$ obtained from simulations compared to the model in \eqref{eq:expectation_test_fct_age} with $\varphi$ being the identity function for $I_{\max}=20$ and $\mu=1$.}
%  \label{fig:mean_age_anytime_I_20}
%\end{figure}
%
%\begin{figure}
%  \centering
%  \includegraphics[width=\linewidth]{./simulations/matlab/fig/quantile_age_at_anytime_mu1_lambdastart0.1_lambdaend2_nr_lambda20_max_msgs20_log_trace_len5.eps}
%  \caption{Quantiles of the age $P[X>x_{\varepsilon}]=\varepsilon$ obtained from integrating the age density in \eqref{eq:f_age_fct_of_pdf_at_arrival} for $I_{\max}=20$ and $\mu=1$.}
%  \label{fig:quantile_age_anytime_I_20}
%\end{figure}




